Personalized and Private Peer-to-Peer Machine Learning

The rise of connected personal devices together with privacy concerns call for machine learning algorithms capable of leveraging the data of a large number of agents to learn personalized models under strong privacy requirements. In this paper, we introduce an efficient algorithm to address the above problem in a fully decentralized (peer-to-peer) and asynchronous fashion, with provable convergence rate. We show how to make the algorithm differentially private to protect against the disclosure of information about the personal datasets, and formally analyze the trade-off between utility and privacy. Our experiments show that our approach dramatically outperforms previous work in the non-private case, and that under privacy constraints, we can significantly improve over models learned in isolation.

==> acks.tex <==
\textbf{Acknowledgments.} This work was partially supported by grant ANR-16-CE23-0016-01, by a grant from CPER Nord-Pas de Calais/FEDER DATA Advanced data science and technologies 2015-2020 and by European ERC Grant 339539 - AOC.


==> background.tex <==
%!TEX root = aistats18_CDPrivacy.tex

% \marc{Maybe, not sure, just a suggestion... gather in section 2 the problem formulation and the privacy framework we work with. Then Section 3, related work, and the contrib starting in Sect 4...}
% \aurelien{i am not convinced: the related work section would then be small and again be split into two parts..}
\section{Preliminaries and Background}
\label{sec:back}

We start by describing the decentralized collaborative learning framework that we consider in this paper, and then review the notion of differential privacy.

\subsection{Problem Setting}

Consider a set of $n$ agents. Each agent $i$ has a local data distribution $\mu_i$ over the space $\mathcal{X}\times\mathcal{Y}$ and has access to a set $\mathcal{S}_i=\{(x_i^j,y_i^j)\}_{j=1}^{m_i}$ of $m_i\geq 0$ training examples drawn i.i.d. from $\mu_i$. The goal of agent $i$ is to learn a model $\theta\in\R^p$ with small expected loss $\myexp_{(x_i,y_i)\sim\mu_i}[\loss(\theta;x_i,y_i)]$, where the loss function $\loss(\theta;x_i,y_i)$ is convex in $\theta$ and measures the performance of $\theta$ on data point $(x_i,y_i)$. In a setting where agent $i$ must learn on its own, the standard approach is to select the model minimizing the local (potentially regularized) empirical loss:
\begin{equation}
\label{eq:solitary}
\theta^{\loc}_i \in \argmin_{\theta\in\R^p} \Big[\underbrace{\frac{1}{m_i}\sum_{j=1}^{m_i} \loss(\theta; x_i^j,y_i^j) + \lambda_i\|\theta\|^2}_{\Loss_i(\theta; \mathcal{S}_i)}\Big],
\end{equation}
with $\lambda_i\geq 0$.
In this paper, agents do not learn in isolation but rather participate in a decentralized peer-to-peer network over which they can exchange information. Such collaboration gives them the opportunity to learn a better model than \eqref{eq:solitary}, for instance by allowing some agents to compensate for their lack of data.
Formally, let $G=(\intset{n},E,W)$ be a weighted connected graph over the set of agents where $E\in\intset{n}\times\intset{n}$ is the set of edges and $W\in\R^{n\times n}$ is a nonnegative weight matrix. $W_{ij}$ gives the weight of edge $(i,j)\in E$ with the convention that  $W_{ij}=0$ if $(i,j)\notin E$ or $i=j$. Following previous work \citep[see e.g.,][]{Evgeniou2004a,Vanhaesebrouck2017a}, we assume that the edge weights reflect a notion of ``task relatedness'': the weight $W_{ij}$ between agents $i$ and $j$ tends to be large if the models minimizing their respective expected loss are similar. These pairwise similarity weights may be derived from user profiles (e.g., in the health domain: weight, size, diabetes type, etc.) or directly from the local datasets, and can be computed in a private way \citep[see e.g.,][]{Goethals2004a,alaggan:hal-00646831}.
% We aim to leverage this assumption to allow agents to collaborate in order to learn a better model than the one they can learn in isolation by simply minimizing their (potentially regularized) empirical local loss:
% \begin{equation}
% \label{eq:solitary}
% \theta^{\loc}_i \in \argmin_{\theta\in\R^p} \Big[\Loss_i(\theta; \mathcal{S}_i) = \frac{1}{m_i}\sum_{j=1}^{m_i} \loss_i(\theta; x_i^j,y_i^j) + \lambda_i\|\theta\|^2\Big], \text{with } \lambda_i\geq 0 \text{ for all } i\in\intset{n}.
% \end{equation}

In order to scale to large networks, our goal is to design \emph{fully decentralized algorithms}: each agent $i$ only communicates with its neighborhood $\Nei{i}=\{j : W_{ij}>0\}$ without global knowledge of the network, and operates without synchronizing with other agents across the network.
Overall, the problem can thus be seen as a multi-task learning problem over a large number of tasks (agents) with imbalanced training sets, and which must be solved in a fully decentralized way.

% \textbf{Relevant work.} Most of the work in decentralized learning and optimization has focused on the distributed consensus problem, where the goal is to find a single global model which minimizes the sum of the local loss functions (see e.g., \cite{Nedic2009a,Ram2010a,Duchi2012b,Wei2012a,Colin2016a}. For decentralized learning of personal models, \cite{Vanhaesebrouck2017a} considered a general objective function which trades off between models with small empirical local loss and models that are smooth within neighborhoods (see Eq.~\ref{eq:Qunified} in Section~\ref{sec:cd_algo}). At the cost of introducing many auxiliary variables, they are able to cast the objective as a partial consensus problem over the network which can be solved using a decentralized gossip ADMM algorithm \cite{Wei2013a}. It involves minimizing a perturbed version of the local loss of two neighboring agents at each iteration $t$ and has an $O(1/t)$ convergence rate.
%They also propose a simpler gossip algorithm for propagating and smoothing the pre-trained local models \eqref{eq:solitary}, which provably converges in expectation but without an explicit convergence rate.
% Privacy constraints were not considered in this work.

% In this work, we propose a simpler broadcast-based block coordinate descent algorithm for the general objective function, which converges faster for strongly-convex loss functions. Furthermore, we design schemes to ensure that users do not leak sensitive information about their data to others while guaranteeing that the learned models remain useful. We rely on the framework of differential privacy, described below.

% In this work, we will (i) propose a simpler and faster broadcast-based block coordinate descent algorithm for the general objective function, and (ii) design privacy-preserving schemes to guarantee that the proposed algorithm does not leak sensitive information about a user's dataset to other users in the network. For the latter, we will rely on the framework of differential privacy, described below.

\subsection{Differential Privacy}
\label{sec:dp}

Differential Privacy (DP) \citep{Dwork2006a} has emerged as a powerful measure of how much information about any individual entry of a dataset is contained in the output of an algorithm.
Formally, let $\mathcal{M}$ be a randomized mechanism taking a dataset as input, and let $\epsilon>0,\delta\geq 0$. We say that $\mathcal{M}$ is $(\epsilon,\delta)$-differentially private if for all datasets $\mathcal{S}=\{z_1,\dots,z_i,\dots,z_m\},\mathcal{S}'=\{z_1,\dots,z'_i,\dots,z_m\}$ differing in a single data point and for all sets of possible outputs $\mathcal{O}\subseteq\range(\mathcal{M})$, we have:
\begin{equation}
\label{eq:dp}
Pr(\mathcal{M} ( \mathcal{S}) \in \mathcal{O}) \leq e^{\epsilon}Pr(\mathcal{M} ( \mathcal{S}') \in \mathcal{O}) + \delta,
\end{equation}
where the probability is over the randomness of the mechanism. At a high level, one can see \eqref{eq:dp} as ensuring that $\mathcal{M} ( \mathcal{S})$ does not leak much information about any individual data point contained in $\mathcal{S}$.
DP has many attractive properties: in particular it provides strong robustness against background knowledge attacks and does not rely on computational assumptions. The composition of several DP mechanisms remains DP, albeit a graceful degradation in the parameters  \citep[see][for strong composition results]{boosting,composition}. We refer to \citet{Dwork2014a} for more details on DP.

% \textbf{Relevant work.} DP has been mostly considered in the context where a ``trusted curator'' has access to all data. Existing DP schemes for machine learning in this setting typically rely on the addition of appropriately scaled noise to the learned model (output perturbation) or to the objective function itself (objective perturbation), see for instance \cite{regularized}.
% The private multi-party setting, in which sensitive datasets are distributed across multiple data owners, is known to be harder \cite{McGregor2010a} and has been less studied in spite of its relevance for many applications.
% Local DP \cite{Duchi2012b,Kairouz2016a}, consisting in locally perturbing the data points themselves before releasing them, often achieves poor accuracy (especially when local datasets are small). An alternative strategy is to rely on DP aggregation of models locally trained by each party \cite{Pathak2010a,Hamm2016a}. DP schemes for (stochastic) gradient descent in the distributed setting have also been proposed, based on perturbing the gradients, the iterates and/or the objective \cite{Song2013a,Rajkumar2012a,Huang2015a,Shokri2015a}.
% Apart from local DP, the above methods do not apply to our setting for a combination of reasons. In particular, the local data distribution is different for each party and we learn a personal model for each agent instead of a single global model. Last but not least, we seek an asynchronous and fully decentralized algorithm without any master node to perform aggregation or coordinate the protocol. We are not aware of any previous DP machine learning schemes designed for this setting.

% \aurelien{check/cite Huang paper and Zhang paper (cited in LOCO paper)}
